Conservative Hybrid Automata from Development Artifacts

The verification of cyber-physical systems operating in a safety-critical environment requires formal system models. The validity of the verification hinges on the precision of the model: possible behavior not captured in the model can result in formally verified, but unsafe systems. Yet, manual construction is delicate and error-prone while automatic construction does not scale for large and complex systems. As a remedy, this paper devises an automatic construction algorithm that utilizes information contained in artifacts of the development process: a runtime monitoring specification and recorded test traces. These artifacts incur no additional cost and provide sufficient information so that the construction process scales well for large systems. The algorithm uses a hybrid approach between a top-down and a bottom-up construction which allows for proving the result conservative, while limiting the level of over-approximation.

==> source/abstract.tex <==

The verification of cyber-physical systems operating in a safety-critical environment requires formal system models.
The validity of the verification hinges on the precision of the model: possible behavior not captured in the model can result in formally verified, but unsafe systems.
Yet, manual construction is delicate and error-prone while automatic construction does not scale for large and complex systems.
As a remedy, this paper devises an automatic construction algorithm that utilizes information contained in artifacts of the development process:  a runtime monitoring specification and recorded test traces.
These artifacts incur no additional cost and provide sufficient information so that the construction process scales well for large systems.
The algorithm uses a hybrid approach between a top-down and a bottom-up construction which allows for proving the result \emph{conservative}, while limiting the level of over-ap\-prox\-i\-ma\-tion.
%
%We validate the construction by simulating canonical examples of hybrid automata to obtain execution traces, reconstructing them with the algorithm, and comparing the result against the original.

